Declarative Traffic Engineering for Low-Latency and Reliable Networking

Cloud-Edge applications like industrial control systems and connected vehicles demand stringent end-to-end latency guarantees. Among existing data plane candidate solutions for bounded latency networking, the guaranteed Latency-Based Forwarding (gLBF) approach ensures punctual delivery of traffic flows by managing per-hop delays to meet specific latency targets, while not requiring that per-flow states are maintained at each hop. However, as a forwarding plane mechanism, gLBF does not define the control mechanisms for determining feasible forwarding paths and per-hop latency budgets for packets to fulfil end-to-end latency objectives. In this work, we propose such a control mechanism implemented in Prolog that complies with gLBF specifications, called declarative gLBF (dgLBF). The declarative nature of Prolog allows our prototype to be concise (~120 lines of code) and easy to extend. We show how the core dgLBF implementation is extended to add reliability mechanisms, path protection, and fate-sharing avoidance to enhance fault tolerance and robustness. Finally, we evaluate the system's performance through simulative experiments under different network topologies and with increasing traffic load to simulate saturated network conditions, scaling up to 6000 flows. Our results show a quasi-linear degradation in placement times and system resilience under heavy traffic.

==> code/glbf.tex <==
\begin{figure}[!ht]
\centering
    \begin{codenum}[firstnumber=1, breaklines]
    glbf(Paths, Capacities) :-
        possiblePaths(PPaths, Capacities),
        validPaths(PPaths, Paths).
    
    possiblePaths([P|Aths], Capacities) :-
        findall(FlowId, flow(FlowId, _, _), FlowIds),
        possiblePaths(FlowIds, Capacities, [P|Aths]).
    possiblePaths(_, Capacities) :-
        findall(FlowId, flow(FlowId, _, _), FlowIds),
        possiblePaths(FlowIds, Capacities, []),!,fail.
    
    possiblePaths(FIds, Alloc, Out) :- possiblePaths(FIds, [], Alloc, [], Out).
    possiblePaths([FId|FIds], Alloc, NewAlloc, OldOut, Out) :-
        flow(FId, S, D), reliabilityReqs(FId, _, Rep),
        enoughCandidatePaths(S, D, Rep),
        paths(FId, Rep, Alloc, TmpAlloc, [], OldOut, FOut),
        possiblePaths(FIds, TmpAlloc, NewAlloc, FOut, Out).
    possiblePaths([FId|_], _, [], _, []) :-
        flow(FId, S, D), reliabilityReqs(FId, _, Rep),
        \+ enoughCandidatePaths(S, D, Rep).
    possiblePaths([], Alloc, Alloc, Out, Out).
    
    enoughCandidatePaths(S, D, 1):- candidate(_, S, D, _), !.
    enoughCandidatePaths(S, D, 2) :-
        candidate(PId1, S, D, P1), candidate(PId2, S, D, P2), dif(PId1, PId2),
        intermediateNodes(P1, N1), intermediateNodes(P2, N2), intersection(N1, N2, []), !.
    
    paths(FId, N, Alloc, NewAlloc, PIds, OldOut, Out) :-
        N > 0, N1 is N-1,
        path(FId, Alloc, TmpAlloc, PId, PIds, OldOut, FOut),
        paths(FId, N1, TmpAlloc, NewAlloc, [PId|PIds], [(FId, PId, FOut)|OldOut], Out).
    paths(_, 0, Alloc, Alloc, _, Out, Out).
    \end{codenum}
\vspace{-3mm}
\caption{Main predicates of \toolname.}
\label{code:glbf}
\end{figure}

==> code/output.tex <==
\begin{figure}[!ht]
    \begin{code}[gobble=4]
    \textbf{?- glbf(Output, Alloc).}
    \textbf{\textcolor{Green}{% 99,025 inferences, 0.016 CPU in 0.018 seconds (89% CPU, 6030755 Lips)}}
    Output = [(f1, p3_nStart_nEnd, [nStart, n4, nEnd], 0.95, (7, 27), 3.5), 
             (f2, p1_nStart_n3, [nStart, n1, n3], 0.96, (23, 43), 11.5), 
             (f2, p2_nStart_n3, [nStart, n2, n3], 0.93, (40, 60), 20), 
             (f3, p3_nStart_nEnd, [nStart, n4, nEnd], 0.95, (-3, 17), 0)],
             
    Alloc  = [(n4, nEnd, 13), (nStart, n4, 13), (n2, n3, 10), 
              (nStart, n2, 10), (n1, n3, 10), (nStart, n1, 10)].
    \end{code}
\vspace{-5mm}
\caption{Example Prolog output, using as input the knowledge base in \cref{code:example}.}
\label{code:output}
\end{figure}

==> code/path_valid.tex <==
\begin{figure}[]
\centering
    \begin{codenum}[breaklines]
    path(FId, Alloc, NewAlloc, PId, PIds, Out, (Path, Rel, NewMinB, Delay)) :-
        flow(FId, S, D), reliabilityReqs(FId, ReqRel, _),
        dataReqs(FId, PktSize, _, BitRate, Budget, Th),
        validCandidate(FId, (S,D), PId, Path, PIds, Out),
        MinB is Budget - Th,
        pathOk(Path, MinB, ReqRel, Alloc, PktSize, BitRate, 1, Rel, NewMinB),
        delay(NewMinB, Path, Delay), 
        updateCapacities(Path, BitRate, Alloc, NewAlloc).

    validCandidate(FId, (S,D), PId, CPath, PIds, Out) :- 
        candidate(PId, S, D, CPath), \+ member(PId, PIds),
        pathProtection(CPath, PIds), 
        noFateSharing(FId, CPath, Out).
    
    noFateSharing(FId, CPath, Out) :-
        findall(AFP, (antiAffinity(FId, Fs), member(F, Fs), member((F,_,AFP,_,_), Out)), AFPs),
        noFateSharing(CPath, AFPs).

    noFateSharing(CPath, [AFPath|AFPs]) :- 
        sharedFirstAndLast(CPath, AFPath, C, AF), intersection(C, AF, []), 
        noFateSharing(CPath, AFPs).
    noFateSharing(_, []).
    
    pathProtection(SPD, PIds) :- intermediateNodes(SPD, P), noIntersections(P, PIds).
    
    noIntersections(P, PIds) :- 
        \+ (member(PId, PIds), candidate(PId,_, _, P1), intermediateNodes(P1, FP), 
        intersection(FP, P, [_|_])).
    
    pathOk([S,N|Rest], OldMinB, ReqRel, Alloc, PktSize, BitRate, OldRel, NewRel, NewMinB) :-
        link(S, N, TProp, Bandwidth, FeatRel),
        reliabilityOk(OldRel, FeatRel, ReqRel, TmpRel),
        hopOk(N, TProp, Bandwidth, Alloc, PktSize, BitRate, OldMinB, TmpMinB),
        pathOk([N|Rest], TmpMinB, ReqRel, Alloc, PktSize, BitRate, TmpRel, NewRel, NewMinB).
    pathOk([_], MinB, _, _, _, _, Rel, Rel, MinB).
        
    hopOK(N, TProp, Bandwidth, Alloc, PktSize, BitRate, MinB, NewMinB) :- 
        node(N, MinNodeBudget), usedBandwidth(N, _, Alloc, UsedBW), 
        Bandwidth > UsedBW + BitRate,
        transmissionTime(PktSize, Bandwidth, TTime),
        NewMinB is MinB - MinNodeBudget - TProp - TTime.

    reliabilityOk(PathRel, FeatRel, ReqRel, NewPathRel) :- 
        NewPathRel is PathRel * FeatRel, 
        NewPathRel >= ReqRel.

    delay(PMinB, [(_,_)], Delay) :- Delay is PMinB, !.
    delay(PMinB, Path, Delay) :- PMinB > 0, length(Path, Hops), Delay is PMinB/Hops.
    delay(PMinB, _, 0) :- PMinB < 0.
    \end{codenum}
\vspace{-3mm}
\caption{Path validation.}
\label{code:path}
\end{figure}

==> code/solution_valid.tex <==
\begin{figure}[]
\centering
    \begin{codenum}[breaklines]    
    validPaths(PPaths, Paths) :-
        findall((F,P,Path), member((F,P,(Path,_,_,_)),PPaths), Paths2),
        compatiblePaths(PPaths, Paths2, Paths).
    
    compatiblePaths([(FId, (P,MinB,D))|Fs], Paths, [(FId, (P, (MinB,MaxB), D))|NewFs]) :-
        flow(FId, _, _, PktSize, BurstSize, _, _, Th),
        totQTime(P, FId, PktSize, BurstSize, Paths, TotQTime),
        MaxB is MinB + 2*Th - TotQTime,  MaxB >= 0,
        compatiblePaths(Fs, Paths, NewFs).
    compatiblePaths([], _, []).
    \end{codenum}
\vspace{-3mm}
\caption{Solution validation.}
\label{code:solution}
\end{figure}
